MobileARLoc: On-device Robust Absolute Localisation for Pervasive Markerless Mobile AR

Recent years have seen significant improvement in absolute camera pose estimation, paving the way for pervasive markerless Augmented Reality (AR). However, accurate absolute pose estimation techniques are computation- and storage-heavy, requiring computation offloading. As such, AR systems rely on visual-inertial odometry (VIO) to track the device's relative pose between requests to the server. However, VIO suffers from drift, requiring frequent absolute repositioning. This paper introduces MobileARLoc, a new framework for on-device large-scale markerless mobile AR that combines an absolute pose regressor (APR) with a local VIO tracking system. Absolute pose regressors (APRs) provide fast on-device pose estimation at the cost of reduced accuracy. To address APR accuracy and reduce VIO drift, MobileARLoc creates a feedback loop where VIO pose estimations refine the APR predictions. The VIO system identifies reliable predictions of APR, which are then used to compensate for the VIO drift. We comprehensively evaluate MobileARLoc through dataset simulations. MobileARLoc halves the error compared to the underlying APR and achieve fast (80\,ms) on-device inference speed.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Sections/5UserStudy.tex <==
\section{Real-life Experiment}

We evaluate \sysname through a user study conducted on the Church scene (Section~\ref{subsec:mobileapp}). This experiment aims to demonstrate the reliability of \sysname with uncontrolled user input, and assess how it benefits the user experience through  objective and subjective measures.

\subsection{Methodology}
\label{subsec:methodology}
%Our experimental setup is as follows: 
We invited 15 participants (6M, 9F, aged 21--30) to participate in an AR treasure hunt. 7 participants had no prior experience with AR. Only one was a frequent user. %The experiment takes the form of a virtual treasure hunt in AR. 

Users were given an iPhone 14 Pro Max and hints about the locations of two virtual objects they had to find with the Basic PN application and with \sysname. Figure~\ref{fig:areffect} displays the location of one object for both applications and its GT.
We defined a perimeter of 5 meters around the object. When users stepped within this boundary, they were instructed to start the application and search for the object. After finding the object, 
the users were asked to assess its exact location. They were encouraged to walk around and observe from different viewpoints for this task. %The users are reminded to decide on the exact location of the objects in this process. 
An observer explained the experiment to the participants, measured the time to find the objects and  to determine their locations and collected feedback through questionnaires and interviews.  The observer also showed participants the objects' position GT after for rating accuracy based on their experience. The objects and their location were pseudo-randomized in each task using Latin square design to avoid bias.

% The observer is in charge of explaining the experiment to the participants, measuring the time to find the object and time to determine the location, and collecting the users' feedback through both questionnaires and interviews. Each participant is assigned different objects in each task with the Latin square design to avoid bias.


% To assess their technological literacy, we pose the following question: ``To how much extent are you familiar with mobile AR applications? 1 – It is the first experience with mobile AR applications, 2 – I tried AR applications before, but only rarely, 3 – I have used some AR applications and have some knowledge about them, 4 – I frequently use AR applications and feel confident with advanced usages, 5 – I work in the field of AR". The average technological confidence is 2.625, with scores ranging from 2 to 5, in which 4 people rate 3 and above. It is the first experience with AR applications for 7 users. 

\begin{figure}[!t]
\centering
  \subfigure[Basic PN]{
 \label{fig:subfig:a} %% label for second subfigure
 \includegraphics[width=0.9\linewidth]{figures/apr_church_small.pdf}}
 \subfigure[\sysname (PN$^{vio}$)]{
 \label{fig:subfig:b} %% label for first subfigure
 \includegraphics[width=0.9\linewidth]{figures/ours_church_small.pdf}}
 \subfigure[GT in point cloud]{
 \label{fig:subfig:a} %% label for second subfigure
 \includegraphics[height=0.8in,width=0.3\linewidth]{figures/bunny_gt2.png}}
 \subfigure[GT in image]{
 \label{fig:subfig:b} %% label for first subfigure
 \includegraphics[width=0.3\linewidth]{figures/church_bunny.jpg}}
  \subfigure[Camera trace]{
 \label{fig:subfig:b} %% label for first subfigure
 \includegraphics[width=0.3\linewidth]{figures/trace.png}}
 \caption{AR frames displaying the 3D bunny at the GT pose using Basic PN and \sysname (ours). \sysname displays virtual objects closer to the GT with much less variability than Basic PN. GT of virtual objects (red boxes in (c) and (d)) are given to users for comparison of accuracy after the tasks. (e) The PN pose (red), \sysname (PN$^{vio}$) pose (green) and camera GT (blue) for one task where the user observes and moves around the objects.
 }
 \label{fig:areffect} %% label for entire figure
\end{figure}


At the end of the experiment, the participants completed 2 questionnaires. The first survey assesses the subjective task load regarding mental demand, physical demand, perceived success, and frustration, inspired by the NASA Task Load Index (TLX)~\cite{hart1988development}. The second survey focuses on the general user experience and the perceived accuracy and stability of \sysname compared to Basic PN. Finally, a short interview addressed the reasons behind the participants' responses.

%focusing on both applications individually, and the other raises questions about the overall experience and comparison between the two applications. In the first survey, we evaluate through 4 parameters, namely mental demand, physical demand, perceived success and frustration. We ask the users the following questions, on a scale from 1 to 10, 1 being the lowest: (i) how mentally demanding was the task? (ii) how physically demanding was the task? (iii) how successful were you in accomplishing what you were asked to do? (iv) how insecure, discouraged, irritated, stressed, and annoyed were you? In the second survey, we inquired about preferences for marker or marker-less approaches, the accuracy, stability, and initialization requirements of \sysname compared to Basic PN. Finally, we collected their comprehensive assessment of both applications based on the aforementioned factors.

\subsection{Results}
\label{subsec:result}

\begin{table}[t!]

\caption{Mean and median absolute translation/rotation errors in $m/^\circ$ on the real-life data collected during the user experiment.}
% \setlength{\tabcolsep}{1pt}
% \resizebox{\columnwidth}{!}{

\small
\begin{tabular}{p{5cm}cc} 
 & MEAN & MED\\
\midrule 
Basic PN & 2.17/8.84   &1.71/5.63\\
\midrule 
\sysname (PN$^{vio}$) &\textbf{0.92/4.40}  &\textbf{0.88/3.86}\\
\bottomrule 
\end{tabular}

%}
\label{tab:resultInUse}
\end{table}

\noindent\textbf{Acccuracy and Robustness: } 
During the user study, we collect 841 frames with the corresponding APR prediction, VIO data, and \sysname optimized prediction. 
We derive the GT for these frames with respect to the original dataset using COLMAP. Table~\ref{tab:resultInUse} displays the mean and median absolute error for these frames with Basic PN and \sysname. \sysname reduces the absolute translation and rotation errors by 57.5\% and 50.2\% respectively.
These findings align with our test set results (Section~\ref{sec:exp}) where our framework significantly reduces the errors from the PN outputs in both translation and rotation. Observing the traces in  Figure~\ref{fig:areffect}(e), \sysname (green) effectively corrects major discrepancies from Basic PN (red), maintaining stability and coherence closely with the GT (blue). Even if the frame is of low quality due to featureless or out-of-scene photography, our framework prevents the large errors produced by PN by optimizing with VIO. These findings underline the enhanced accuracy our framework brings to real-world application usage statistically.




% %We collect 841 frames with corresponding data during the completion of 6 different tasks in our user study.
% Reconstructing using COLMAP with a test sequence, we derive GT for the newly captured frames in the original coordinate system, which is consistent with the APR and optimized poses. As depicted in table in table~\ref{tab:resultInUse}, there's a notable reduction in mean absolute translation and rotation errors by 57.5\% and 50.2\% respectively. These findings align with our test set results (Section~\ref{sec:exp}) where our framework significantly reduces the errors from the PN outputs in both translation and rotation. Observing the traces in  Figure~\ref{fig:areffect}(e), \sysname (green) effectively corrects major discrepancies from Basic PN (red), maintaining stable and coherent closely with the GT (blue). Even if the frame is of low quality due to featureless or out-of-scene photography during the process of searching for the objects, our framework manages to prevent large errors produced by PN and optimizes it through VIO. These findings underscore the enhanced accuracy our framework brings to real-world application usage statistically.


\noindent\textbf{Task completion time: } 
Time is measured in 2 stages: (1) once the user entered the perimeter of 5m surrounding the virtual objects, we measured the time until the user declared stable objects were found; (2) we then measured the time for users to assess the exact location of the objects. 
As shown in Figure~\ref{fig:nasa}(b), the average time for finding the stable objects for Basic PN is 25.67 seconds, while for \sysname is 21.47 seconds, including two outliers, namely 51 and 55 seconds. In these two cases, improper operation added extra difficulty to the initialization stage; for example, shooting facing a featureless wall or remaining stable in both position and camera orientation prevented initialization. The average time for users to determine the exact positions of objects is 45.6\,s for Basic PN and 27.53\,s for \sysname. 
Follow-up interviews show that \sysname anchors the virtual objects with little variation over time compared to Basic PN which periodically relocalizes. As such, \sysname nearly halves the decision-making time for determining the object location, which is significant in AR tasks requiring accurate placement of digital objects (e.g., fine-grained interaction).

% \sysname notably elevates the user experience by nearly halving the decision-making time for object location determination while improving accuracy and reliability.


\iffalse
\begin{figure}[t!]
 \centering
   \subfigure[Mental]{
   \centering
 \label{fig:subfig:f} %% label for second subfigure
 \includegraphics[width=.225\linewidth]{figures/boxplot_mental.png}}
 \subfigure[Physical]{
 \centering
 \label{fig:subfig:a} %% label for first subfigure
 \includegraphics[width=.225\linewidth]{figures/boxplot_physical.png}}
    \subfigure[Success]{
   \centering
 \label{fig:subfig:f} %% label for second subfigure
 \includegraphics[width=.225\linewidth]{figures/boxplot_success.png}}
 \subfigure[Frustration]{
 \centering
 \label{fig:subfig:a} %% label for first subfigure
 \includegraphics[width=.225\linewidth]{figures/boxplot_frustration.png}}
 \caption{Boxpolts of (a) mental demand, (b) physical demand, (c) perceived success and (d) frustration for tasks using both applications. The red line represents the median value and the blue one shows the average value. \sysname requires less physical and mental demand than the basic PN, with greater success perceived and less frustration.
 }
 \label{fig:nasa} %% label for entire figure
\end{figure}
\fi

\begin{figure}[!t]
  \centering
  \subfigure[NASA TLX Results]{
   \centering
 \label{fig:subfig:f} %% label for second subfigure
 \includegraphics[width=.45\linewidth]{figures/tlx.pdf}}
 \subfigure[Task completion time]{
 \centering
 \label{fig:subfig:a} %% label for first subfigure
 \includegraphics[width=.45\linewidth]{figures/task_time_interval.pdf}}
\caption{(a) Boxpolts of mental demand, physical demand, perceived success and frustration (blue: Basic PN; orange: \sysname). The red line represents the median value. \sysname requires less physical and mental demand than the basic PN, with greater success perceived and less frustration. 
(b) Average task completion time for \sysname and Basic PN. 
%\sysname almost halves the time for users to determine the locations of virtual objects.
 }
\label{fig:nasa}
\end{figure}

\noindent\textbf{Survey: } 
Figure~\ref{fig:nasa}(a) showcases the perceived task load in terms of mental demand, physical demand, perceived success, and frustration for both applications. We assess statistical significance with Student's t-test for repeated measures. There is a statistically significant difference ($p<0.05$) between in  mental demand. Unsurprisingly, there is little difference in physical demand as both tasks demanded the same amount of motion. Finally, although \sysname displays visibly higher perceived success and lower frustration, the wide variance does not show a statistically significant difference.

% %However, according to our question in the second survey, more participants are still in favor of marker-less approaches than marker-based ones. 
% For perceived success, \sysname also has higher average (5.07) and median (5) score, outperforming Basic PN (avg=4.27, med=4). 
% %and the marker-based application (avg=3.87, med=2). 
% %Some participants convey that marker-less applications offer more practicality in day-to-day settings and deliver a delightful element of surprise. The greater sense of accomplishment may also be the reason for more perceived success. 
% The frustration for \sysname has a low variance: 9 people experience low frustration ($\leq3$), only 1 user reports high levels of frustration ($\geq7$). On the contrary, 8 users experience low frustration and 4 display high frustration in Basic PN. In summary, our framework substantially enhances the mobile AR experience.

% \begin{figure}[htb!]
%  \centering
%    \subfigure[Stability $\&$ Robustness]{
%    \centering
%  \label{fig:subfig:f} %% label for second subfigure
%  \includegraphics[width=.45\linewidth]{figures/bar_stability.png}}
%  \subfigure[Task completion time]{
%  \centering
%  \label{fig:subfig:a} %% label for first subfigure
%  \includegraphics[width=.45\linewidth]{figures/bar_task_time2.png}}
%  \caption{(a) Plots of users rating from 1-5 to compare \sysname with Basic PN in terms of stability and robustness. 1 means \sysname to be less stable than Basic PN, 3 means moderate performance and 5 means more stable. Only 3 users rated \sysname to be less stable than Basic PN. (b) Average task completion time for marker-less approaches. \sysname improves the efficiency for users to identify and locate the objects.
%  }
%  \label{fig:comparison} %% label for entire figure
% \end{figure}

% \begin{figure}[htb!]
%  \centering
%    \subfigure[Stability $\&$ Robustness]{
%    \centering
%  \label{fig:subfig:f} %% label for second subfigure
%  \includegraphics[width=.45\linewidth]{figures/bar_stability.png}}
%  \subfigure[Task completion time]{
%  \centering
%  \label{fig:subfig:a} %% label for first subfigure
%  \includegraphics[width=.45\linewidth]{figures/bar_task_time2.png}}
%  \caption{(a) Plots of users rating from 1-5 to compare \sysname with Basic PN in terms of stability and robustness. 1 means \sysname to be less stable than Basic PN, 3 means moderate performance and 5 means more stable. Only 3 users rated \sysname to be less stable than Basic PN. (b) Average task completion time for marker-less approaches. \sysname improves the efficiency for users to identify and locate the objects.
%  }
%  \label{fig:comparison} %% label for entire figure
% \end{figure}


\iffalse
\begin{figure}[t]
 \centering
 \includegraphics[width=.45\linewidth]{figures/bar_task_time2.png}
 \caption{Average task completion time for \sysname and Basic PN. \sysname almost halves the time for users to assess the exact location of the virtual objects.
 }
 \label{fig:robust} %% label for entire figure
\end{figure}
\fi

% \begin{table}[hbt!]
% \caption{The overall experience based on their performance and limitations from 1 to 10. 1 means very bad and 10 means very good.}
% \setlength{\tabcolsep}{1pt}
% \resizebox{\columnwidth}{!}{
% $$
% \begin{tabular}{c|ccccc} 
% \text{Overall experience based on performance $\&$ limitations} & \text{AVG} & \text{MED} & \text{MIN} & \text{MAX} & \text{STDEV}\\
% \hline 
% \text{Basic PN} &\text{4.93} &\text{6} &\text{1} &\text{7} &\text{2.28}\\
% \hline 
% \text{\sysname (PN$^{vio}$)} &\text{7.33} &\text{8} &\text{2} &\text{10} &\text{2.47} \\
% \hline 
% \end{tabular}
% $$
% }
% \label{tab:survey2}
% \end{table}

\begin{table}[t!]
\caption{Overall experience, perceived accuracy, and perceived robustness ranked from 1 to 5. Higher is better.}
% \setlength{\tabcolsep}{1pt}
% \resizebox{\columnwidth}{!}{
% $$
\small
\begin{tabular}{p{3cm}C{0.5cm}C{0.5cm}C{0.5cm}C{0.5cm}C{0.5cm}C{0.5cm}} 
 & \multicolumn{2}{c}{User Exp.} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{Robustness} \\
 \cmidrule{2-7}
 & AVG & MED & AVG & MED & AVG & MED\\
\midrule 
Basic PN & 2.47 & 3 & 2.53 & 2 & 2.13 & 1\\
\midrule 
\sysname (PN$^{vio}$) &\textbf{3.67} &\textbf{4} &\textbf{3.47} &\textbf{4} &\textbf{3.87} & \textbf{5} \\
\bottomrule 
\end{tabular}
% $$
% }
\label{tab:survey2}
\end{table}

The second survey concentrates on comparing stability and robustness between Basic PN and \sysname.   Table~\ref{tab:survey2} presents the average and median user experience, perceived accuracy, and robustness for each application.
Most users believe \sysname offers a more accurate (9 participants) and robust (10 participants) experience. Similarly, participants rate their overall experience close to 50\% higher with \sysname compared to Basic PN. Student t-test for repeated measures shows a statistically significant difference for all measures ($p<0.05$). 
The high difference between average and median comes from a small sample of participants that took the experiment in extreme sunny conditions, resulting in overexposure of camera frames which affected both the APR and ARKit's VIO, leading to poor performance. Overall, our framework significantly improves the performance in finding virtual objects in terms of accuracy and reliability. 

% In addition, we conduct a paired-sample t-test against the null hypothesis concerning the overall experience. The results suggest that \sysname offers a superior user experience, with T = 2.60 and P = 0.02.


%  % The second survey concentrates on drawing comparisons between the applications. 
% Figure~\ref{fig:comparison}.a visualizes the ratings rating from 1-5 for stability. 
% A significant majority of users believe \sysname offers superior stability compared to the Basic PN. To statistically validate the difference in the reliability difference between the two applications, we conducted a paired-sample t-test. This test is against the null hypothesis, which posits that the paired data samples share the same mean. The result indicates that \sysname offers a more stable experience to the users (T = 2.16, P \textless \ 0.05). Similarly for the comparison of accuracy, 5 users think \sysname more accurate than Basic PN, 1 thinks less accurate and 9 perceive little difference or consider them identical. Moreover, 66.7\% of users think that the initialization stage in our framework doesn't have much influence. Among them, 30\% users choose ``None influential at all". In table~\ref{tab:survey2}, \sysname has a significant rise in the average and median score for the overall experience considering performance and limitations. In addition, we conduct a paired-sample t-test against the null hypothesis concerning the overall experience. The results suggest that \sysname offers a superior user experience, with T = 2.60 and P = 0.02.
 %Notably, the marker-based method achieve the highest score, attributed largely to its streamlined object detection process and inherent robustness due to the utilization of markers. However, most people believe whether to use markers or not are two different cases in the interview. Although markers can provide a better user experience, it's impractical in some scenarios where marker-less approaches can take advantage.

 %We also shed light on the impracticality of markers through greater perceived success from \sysname and user preference for marker-less methods.










\subsection{Findings and discussion}
\label{subsec:finding}

\noindent\textbf{Summary of Findings: } 

The experiment presents the following findings:
\begin{enumerate}
    \item \sysname significantly improves the user experience of marker-less mobile AR in accuracy and reliability, with less physical, mental demand and frustration.
    %\item While the vast majority of users think the performance of marker-based method surpasses that of \sysname and Basic PN, more users still express a preference for marker-less approaches over the marker-based one. As from the interview, users believe that the choice between the two depends on scenarios. Moreover, the marker-less method is perceived to be more suitable for daily use, bringing added enjoyment and a heightened sense of achievement.
    \item Task completion time is uncorrelated with the technological literacy. With \sysname, the completion time is reduced because users find it more intuitive. Unlike Basic PN, virtual objects in \sysname don't drift extensively or frequently.
    \item \sysname is an APR-agnostic framework with low computation overhead and energy consumption, which users intend to use in the future.
\end{enumerate}

\noindent\textbf{Discussions: } 
Our framework shows improved accuracy and reliability compared to applications that directly use output from an APR model, resulting in a more seamless user experience. 66.7\% of users don't perceive the initialization period to be influential. However, in two cases, improper operations like shooting facing a featureless wall or remaining stable in both position and camera orientation added extra difficulty to initialization. 
% It's crucial to understand AR applications are not one-shot scenarios, and we aim to provide a better experience instead of frequent alignment at the very beginning. 
An alternative to the initialization period can be directly using the APR output for scenarios where immediateness is more important than initial accuracy, including robotics and navigation, and refining over time. 

% At the end of the experiment, we provide a marker-based demo using Vuforia SDK~\footnote{https://developer.vuforia.com/} to display the objects. Although the vast majority of users think the performance of the marker-based method surpasses that of \sysname and Basic PN, more users still prefer marker-less approaches over the marker-based one. They believe whether to use markers or not are two different cases in the interview. Although markers can provide a better user experience, it's impractical in some scenarios where marker-less approaches can take advantage. Moreover, the marker-less method is perceived to be more suitable for daily use, bringing added enjoyment and a heightened sense of achievement.


